Live Programming for Finite Model Finders

Finite model finders give users the ability to specify properties of a system in mathematical logic and then automatically find concrete examples, called solutions, that satisfy the properties. These solutions are often viewed as a key benefit of model finders, as they create an exploratory environment for developers to engage with their model. In practice, users find less benefit from these solutions than expected. For years, researchers believed that the problem was that too many solutions are produced. However, a recent user study found that users actually prefer enumerating a broad set of solutions. Inspired by a recent user study on Alloy, a modeling language backed by a finite model finder, we believe that the issue is that solutions are too removed from the logical constraints that generate them to help users build an understanding of the constraints themselves. In this paper, we outline a proof-of-concept for live programming of Alloy models in which writing the model and exploring solutions are intertwined. We highlight how this development environment enables more productive feedback loops between the developer, the model and the solutions.

==> casestudy.tex <==
\section{Case Study}\label{sec:casestudy}

==> eval.tex <==
\section{Evaluation}\label{sec:eval}
We evaluate \tool{} in two ways. First, we evaluate the overhead of translating graphical renderings into executable test cases. Second, we conduct an illustrative case study over a select set of models to highlight how \tool{} can ease the burden of creating test cases for models with tedious features for textual test case creation. 

\subsection{Overhead} 
Table~\ref{tab:overhead} shows the runtime to translate the canvas state of \tool{} into a command string for increasingly larger and larger test cases. Column \textbf{Model} conveys the model under evaluation. The next two columns outline the size of the model: column \textbf{\#Sig} is the number of signatures and column \textbf{\#Rel} is the number of relations in the model. To convey the size of the test case, column \textbf{\#Atoms} displays the number of atoms on the canvas and column \textbf{\#Con} shows the number of connections on the canvas. Column \textbf{Time[s]} conveys the time it takes for \tool{} to generate the command string once the execute test button in pressed. To perform the calculations, we create incrementally larger graphical test cases in \tool{} for the two models we explore in our case study: the LTS model, which contains a higher arity relation, and the CV model, which contains a large number of signature and relations.

\subsection{Case Study: Debugging Real World Faulty Models}
For our case study, we focus on two models from the Alloy4Fun benchmark~\cite{alloy4funbenchmark}. Alloy4Fun is a online learning platform for Alloy whose exercises have users attempt to write predicates for various models, which are checked against a back-end oracle solution. Submissions to Alloy4Fun have been anonymized and made into an open source benchmark~\cite{alloy4funbenchmark}. These models represent faulty models created by new Alloy users. While AUnit is available for any Alloy user, we envision that new users are more likely to utilize AUnit. Our case study looks to highlight how different model structures can make writing AUnit test cases tedious and error prone.
%: (1)~how an AUnit test case could help the user understand the faulty behavior and (2)~. 

\begin{table}[]
    \centering
    \caption{Overhead of Translation}
    \label{tab:overhead}
    \input{tables/overhead}
\end{table}

\subsubsection{Case Study: Higher Arity Relations}
Often times, Alloy models consist of binary relations (2-arity). For instance, in Figure~\ref{fig:alloy}, the relation \CodeIn{header} is a binary relation of the form \CodeIn{List$\times$Node}. This is conceptually easier for a user to visualize mentally and put to paper, as the \CodeIn{header} can be envisioned a directed line that connects a single \CodeIn{List} atom to a single \CodeIn{Node} atom. However, in Alloy, it is possible for a relation of higher arity to be specified. To illustrate, consider the Labeled Transition System (LTS) model from the Alloy4Fun benchmark shown in Figure~\ref{fig:lts}. Line 1 introduces the signature \CodeIn{State}, which contains the relation \CodeIn{trans}. This relation is a trenary relation (3-arity) of the form \CodeIn{State$\times$Event$\times$State}. Rather than being a directed line between two atoms, \CodeIn{trans} is two chains long, with an intermediate \CodeIn{Event} atom that connects the states. The idea of the \CodeIn{trans} relation is to that the transitions between states are triggered by events; therefore, this intermediate \CodeIn{Event} atom is an important connection between the states. Line 2 introduces the \CodeIn{Init} signature on line 2 as a subset (\CodeIn{in}) of the \CodeIn{State} signature, which conveys the initial state of the system, and line 3 introduces the signature \CodeIn{Event} that contains no relations itself. The faulty predicate \CodeIn{inv3} (lines 6 - 8) is meant to convey that the LTS is deterministic, meaning that for every state, every \CodeIn{Event} triggers either no transition or a unique transition to a next state. We elect to illustrate \tool's experience over predicate \CodeIn{inv3}, which is the third exercise in the LTS model on Alloy4Fun, as it involves the \CodeIn{trans} ternary relation in its formulation. The following is the correct version of the predicate:

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
\Blue{all} s : State, e : Event | \Blue{lone} \Red{e}.(\Red{s}.trans)
\end{Verbatim}
\end{footnotesize}

The incorrect version swaps the relations on which the relational joins are applied. This error is a subtle change textually, but the fault results in a formula that is trivially \textit{always} true. Namely, ``\CodeIn{e.trans}'' looks to form a relational join of the form \CodeIn{Event} with \CodeIn{State->Event->State}. Since there is a type mismatch between \CodeIn{Event} and \CodeIn{State}, this first join will always be empty. To reveal this fault, the user needs to be an AUnit test case in which an \CodeIn{Event} triggers multiple possible state transitions for the same state. Textually, the following is a test case that reveals this fault: % For an end user building a test case, the user may realistically want to check that each transition out of a given state to a new state has a unique event that triggers it by intentionally creating a test case where this is not true.


\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
State = State0 + State1
trans = \Red{State1->Event0}->State0 
      + \Red{State1->Event0}->State1 
Event = Event0 + Event1 + Event2
 Init = State1
\end{Verbatim}
\end{footnotesize}

%  + State1->Event1->State0 + State1->Event1->State1 
%  + State1->Event2->State0 + State1->Event2->State1

\noindent where the red text helps highlight the faulty behavior. For comparison, Figure~\ref{fig:ltscrucible} (a) displays the same test case recreated in \tool. \Fix{add screenshot} To illustrate how these two \CodeIn{trans} relations are problematic, consider the evaluation of the expression correct sub-expression ``\CodeIn{State1.trans}'' and the faulty sub-expression ``\CodeIn{Event0.trans}'' over the test case:

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
State1.trans = Event0->State0 + Event0->State1 
Event0.trans = \{\}
\end{Verbatim}
\end{footnotesize}
%             + Event1->State0 + Event1->State1 
%             + Event2->State0 + Event2->State1

\noindent Then, if we expanded both of these expression out to the correct expression ``\CodeIn{Event0.(State1.trans)}'' and the faulty expression ``\CodeIn{State1.(Event0.trans)}'', we get to the following:

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
Event0.State1.trans = State0 + State1 
State1.Event0.trans = \{\}
\end{Verbatim}
\end{footnotesize}

\noindent which reveals that the constraint ``\CodeIn{lone} e.(s.trans)'' is false when \CodeIn{e} is \CodeIn{Event0} and \CodeIn{s} is \CodeIn{State1} but ``\CodeIn{lone} s.(e.trans)'' is true for the same variables.  As the above outlines, it is feasible to create a fault revealing test case textually. However, since the relations are higher arity, it is also easy to accidentally make an error, especially for larger test cases where the user may realistically copy, paste and tweak assignments to the \CodeIn{trans}.  For example, the following \CodeIn{trans} relation can extend our fault revealing test case:

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
State = State0 + State1 + State2
trans = State0->Event0->State0 + State0->Event0->State1 
      + State0->Event0->State2 + State0->Event1->State0 
      + State0->Event1->State1 + State0->Event1->State2 
      + State0->Event2->State0 + State0->Event2->State1 
      + State0->Event2->State2 + State1->Event0->State0 
      + State1->Event0->State1 + State1->Event0->State2 
      + State1->Event1->State0 + State1->Event1->State1 
      + State1->Event1->State2 + State1->Event2->State0 
      + State1->Event2->State1 + State1->Event2->State2 
      + State2->Event0->State0 + State2->Event0->State1 
      + State2->Event0->State2 + State2->Event1->State0 
      + State2->Event1->State1 + State2->Event1->State2 
      + State2->Event2->State0 + State2->Event2->State1 
      + State2->Event2->State2
Event = Event0 + Event1 + Event2
 Init = State1
\end{Verbatim}
\end{footnotesize}

\noindent which is significantly harder to follow textually. The extension to this test case is derived by using Amalgam~\cite{Amalgam} to create a maximal scenario based on the first test case. Using Amalgam allows us to highlight one of the largest, and as a result one of the more complex, fault revealing AUnit test case that a user could, in theory, create based on the current scope that preserves the same general fault revealing constraints as the smaller initial test case. If a user is looking to perform fault localization, repair or partial model synthesis with their AUnit test suite, past experiments reveal that larger test cases that encompass a wide degree of behavior result is notably better performance for these frameworks~\cite{AlloyFL,ARepair,ASketchABZ}. As a result, a user is, in general, motivated to create more intricate test cases over smaller, and likely more narrow, test cases.
%If the user is intentionally trying to create the expected invalid behavior with the two \CodeIn{State1->Event0} transitions but wants to create a large test case t, it is easy to see how a user may accidentally introduce some other mistake along the way that could obscure this behavior.
In addition, if the user is textually specifying a relation as large as the \CodeIn{trans} relation outlined above, the user would realistically execute the test case and visually inspect the scenario the Analyzer produces to make sure the valuation matches there expectation. \tool{} removes the need to do these types of ad-hoc validations for AUnit test cases. To illustrate, Figure~\ref{fig:ltscrucible} (b) displays this same larger test case recreated in \tool. \Fix{Add screenshot.} Since \tool{} provides a live graphical view as the user builds up a test case, the main advantage of using \tool{} to create test cases for models with high arity relations is that \tool{} can directly reduce the burden of mentally picturing long text chain for specifying a test case.

\begin{figure}
    \centering
    \input{figures/lts}
    \caption{Faulty Model of a Labeled Transition System (LTS)}
    \label{fig:lts}
\end{figure}



\subsubsection{Case Study: Numerous Signatures and Relations}
In a recent profile of over 2000 different Alloy models~\cite{staticprofilealloy}, the predominate number of signatures and relations that appear in models is 2 each, which was measured as the most recurring value. However, that same study found that the typical use, the median number, of signatures and relations is 8 and 2 respectively. Therefore, while it is possible for an Alloy model to have a small number of signatures and relations, it is equally possible that a user is working with a large number of signatures and relations. As the number of signatures and relations grow, the complexity of the valid scenarios for the models also grows. While Alloy defaults to a scope of 3 for commands, this scope is an upper bound of the size of \emph{each} signature individually, and not a collectively shared scope. As a result, if a user has 8 signatures in their model, a valid scenario can have up to 24 atoms. In addition, the scope does not place any restrictions on the size of relations. Therefore, these 24 atoms can be interconnected in 10s or even 100s of ways. All of this increases the burden for a user to mentally visualize a scenario and then textually specify the corresponding test case. In fact, it would not be surprising in this instance, if the user first drew a scenario on paper before writing the corresponding test case. 

To illustrate how \tool{} can ease the burden of creating test cases with numerous signatures and relations, we select the \CodeIn{CV} model from the Alloy4Fun benchmark, which has 5 signatures and 4 relations, as seen in Figure~\ref{fig:cv}. Line 1 introduces an abstract signature \CodeIn{Source}. As an abstract signature, \CodeIn{Source} cannot directly have atoms itself. The next two signatures extend the \CodeIn{Source} signature. Line 2 introduces the signature \CodeIn{User}, which contains two relations: \CodeIn{profile} connects a \CodeIn{User} to any number (\CodeIn{set}) of \CodeIn{Work} elements (line 3) and \CodeIn{visible} connects a \CodeIn{User} to any number (\CodeIn{set}) of \CodeIn{Work} elements as well (line 4). Line 6 introduces the signature \CodeIn{Institution} and line 8 introduces the signature \CodeIn{Id}, neither of which define any relations. Lastly, line 9 introduces the signature \CodeIn{Work} , which contains two relations: \CodeIn{ids} connects a \CodeIn{Work} atom to at least one (\CodeIn{some}) \CodeIn{Id} atom (line 10) and \CodeIn{source} connects a \CodeIn{Work} atom to exactly one (\CodeIn{one})  \CodeIn{Source} atom (line 11). The faulty predicate \CodeIn{inv1} (lines 16 - 18) attempts to use subset (\CodeIn{in}) to specify that any visible work is someone's CV must be part of that person's profile. The correct version of the predicate is: 

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
\Blue{all} u:User | u.visible \Blue{in} u.profile 
\end{Verbatim}
\end{footnotesize}

\noindent which is similar to the incorrect formula, but constrains the subset relationship to be true for each individual person (\CodeIn{\Red{u}.visible}), instead of a universal perspective (\CodeIn{\Red{User}.visible}). As a result, for the incorrect formula, a user could have a visible work in their CV as long as at least one person has that work in their profile, even if that person it not them. Consider the following fault revealing test case: 

\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
 Source = User0 + User1
   User = User0 + User1
profile = \Red{User1}->Work0 + \Red{User1}->Work1 + \Red{User1}->Work2
visible = \Red{User0}->Work0 + \Red{User0}->Work1 + \Red{User0}->Work2
     Id = Id0
   Work = Work0 + Work1 + Work2
    ids = Work0->Id0 + Work1->Id0 + Work2->Id0
 source = Work0->User1 + Work1->User1 + Work2->User0
\Blue{no} Institution
\end{Verbatim}
\end{footnotesize}

The issue with this test case is that \CodeIn{User0} is able to have \CodeIn{Work0} visible on their CV despite not having \CodeIn{Work0} in their profile because another user (\CodeIn{User1}) has the work in their profile. In fact, for this test case, this is true for every single work that is visible on \CodeIn{User0}'s cv. At first glance, this relationship may be easy to type and confirm textually. However consider the following test case, which is an extension of the previous test case:


\begin{footnotesize}
\begin{Verbatim}[frame=lines,rulecolor=\color{lightgray}]
 Source = User0 + User1 + User2
   User = User0 + User1 + User2
profile = User0->Work1 + User0->Work2 + \Red{User1->Work0}
        + User1->Work1 + User1->Work2 + \Red{User2->Work0} 
        + User2->Work1 + User2->Work2
visible = \Red{User0->Work0} + User0->Work1 + User0->Work2 
        + User1->Work0 + User1->Work1 + User1->Work2 
        + User2->Work0 + User2->Work1 + User2->Work2
    Id = Id0 + Id1 + Id2
   Work = Work0 + Work1 + Work2
    ids = Work0->Id0 + Work0->Id1 + Work0->Id2 
        + Work1->Id0 + Work1->Id1 + Work1->Id2 
        + Work2->Id0 + Work2->Id1 + Work2->Id2
 source = Work0->User2 + Work1->User2 + Work2->User1
\Blue{no} Institution
\end{Verbatim}
\end{footnotesize}

This test case is again derived by using Amalgam to create a maximal scenario based on the first test case~\cite{Amalgam} to also highlight one of the largest fault revealing AUnit test case a user could in theory create based on the scope being explored. Again, the faulty behavior is revealed by the portion presented in red text. Figure~\ref{fig:cvcrucible} displays the same test case recreated in \tool. \Fix{Add screenshot.} As with the LTS model, the main advantage of using \tool{} is reducing the uncertainty of mentally re-creating such a long text chain for specifying a test case. In this case, rather than the majority of the complication being one relation, the complexity comes from the combination of different ways the atoms can relate to one another within the model. However, in both cases, there is a high spatial cognitive burden to attempt to mentally visualize the test valuation.

\begin{figure}
    \centering
    \input{figures/cv}
    \caption{Faulty Model of a Curriculum Vitae Policy}
    \label{fig:cv}
\end{figure}

%\subsection{Case Study: Addr}
%As mentioned in Section~\ref{sec:bg}, one of the difficulties in translating the mental image of a scenario to a textual representation lies in specifying higher arity relations. Figure~\ref{fig:addr} displays a faulty Alloy model of an address book that originated from an Alloy tutorial and a fault revealing AUnit test case~\cite{}. The relation \CodeIn{entry} is a standard binary relation that maps each \CodeIn{Book} object to any number of \CodeIn{Name} objects. In contrast, \CodeIn{listed} is a ternary relation (3-arity) that makes an entry (\CodeIn{Book->Name}) element to any number of \CodeIn{Listing} elements, which can either be \CodeIn{Address} or \CodeIn{Name} elements. Therefore, \CodeIn{listed} takes the form \CodeIn{Book->Name->Listing}. 

%Figure~\ref{fig:arr} displays an Alloy model of an array data structure. The relation \CodeIn{i2e} maps indexes to elements of Element and is a 3-arity relation. In constrast, \CodeIn{length} is a binary relation (2-arity). 
%\begin{figure}
%    \centering
%    \input{figures/arr}
%    \caption{Alloy Model of an Array}
%    \label{fig:arr}
%\end{figure}

%\begin{figure*}
%    \centering
%    \input{figures/addr}
%    \caption{Faulty Alloy Model of an Address Book}
%    \label{fig:addr}
%\end{figure*}

%\subsection{Case Study: Gradebook}
%\begin{figure*}
%    \centering
%    \input{figures/grade}
%    \caption{Alloy Model of a Gradebook Scheme}
%    \label{fig:grade}
%\end{figure*}
